Group-In: Group Inference from Wireless Traces of Mobile Devices

This paper proposes Group-In, a wireless scanning system to detect static or mobile people groups in indoor or outdoor environments. Group-In collects only wireless traces from the Bluetooth-enabled mobile devices for group inference. The key problem addressed in this work is to detect not only static groups but also moving groups with a multi-phased approach based only noisy wireless Received Signal Strength Indicator (RSSIs) observed by multiple wireless scanners without localization support. We propose new centralized and decentralized schemes to process the sparse and noisy wireless data, and leverage graph-based clustering techniques for group detection from short-term and long-term aspects. Group-In provides two outcomes: 1) group detection in short time intervals such as two minutes and 2) long-term linkages such as a month. To verify the performance, we conduct two experimental studies. One consists of 27 controlled scenarios in the lab environments. The other is a real-world scenario where we place Bluetooth scanners in an office environment, and employees carry beacons for more than one month. Both the controlled and real-world experiments result in high accuracy group detection in short time intervals and sampling liberties in terms of the Jaccard index and pairwise similarity coefficient.

==> Deployment.tex <==
\section{Live Deployment}
\label{Section:Deployment}

\begin{figure}
  \includegraphics[width=0.45\textwidth, cfbox=black 0.5pt 0.5pt]{figures/GroupIn.pdf}
\centering
\caption{A view from Group-In's live web interface for the group detection in Gold Coast.} %Top: Number of groups by time, bottom-left: number of people detected by time, bottom-right: group members at the latest time interval.} 
\label{Fig:WebInterface}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.65\columnwidth]{figures/GoldCoastDeployment_Anonym.pdf}
\caption{Locations of the Wi-Fi scanners in Gold Coast.}% (marked with location tags) and 2 cameras.}
\label{Fig:Deployment}
\end{figure}


\begin{table}
\begin{tabular}{@{}lc@{}}
\toprule
\textbf{Pilot data}& \textbf{Info}\\ \midrule
Deployment period& Oct'17 - Dec'18\\
\# Wi-Fi scanners& 17\\
\# Wi-Fi traces  & $\sim$250M\\
Wi-Fi data storage& $\sim$2TB\\
Wi-Fi probe rate (per scanner) & $\sim$100-200Hz \\
Virtual machine (per cluster) & 4 cores, 16GB RAM\\
%\# camera devices   & 2\\
%\# camera counts& $\sim$960K\\
%Camera count message storage&$\sim$7.2GB\\
%Virtual machines   & 4 cores, 16GB RAM\\
%Avg. field test accuracy          & 94\% \\
%Operation availability          & 87\% \\
%Number of field tests    & 12\\
\bottomrule       
\end{tabular}
\caption{Information about the Gold Coast pilot study.}
\label{tab:Deployment}
\end{table}

\begin{table*}[t!]
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    %& \multicolumn{4}{|c|}{Display Format}& \\ \cline{2-5}
    &\multicolumn{3}{|c|}{Cluster 1}& \multicolumn{3}{|c|}{Cluster 2} \\  \hline
    Time interval& \# people & DB query time    & Group detection time& \# people & DB query time & Group detection time \\ \hline
    2 min &  43.09$\pm$7.19& 0.55$\pm$0.18      & 0.75$\pm$1.12 &           2.21$\pm$0.59 &0.05$\pm$0.02          &0.06$\pm$0.03\\ \hline
    5 min & 59.40$\pm$9.39 & 1.28$\pm$0.38      & 1.85$\pm$2.11 &           2.61$\pm$1.05 &0.10$\pm$0.04          &0.12$\pm$0.04\\ \hline
   10 min & 80.85$\pm$14.12& 2.49$\pm$0.67      & 3.97$\pm$3.94 &           3.85$\pm$1.95 &0.18$\pm$0.06          &0.21$\pm$0.07\\ \hline
   30 min & 152.67$\pm$37.21& 7.35$\pm$1.74     & 20.22$\pm$14.64 &         12.46$\pm$5.13 &0.46$\pm$0.15       &0.65$\pm$0.21\\ \hline
   60 min & 231.45$\pm$72.79& 15.51$\pm$3.34    & 79.36$\pm$64.18 &         19.70$\pm$9.36 &0.86$\pm$0.28       &1.42$\pm$0.52\\ \hline
    \end{tabular}
    \caption{Mean and std. values for group detection time and database query time (sec) as a result of the number of people detected in Gold Coast pilot study. Time period: 1.5 months. Sampling time: 30~sec, Cluster 1 with 13 scanners and Cluster 2 with 4 scanners. Applied algorithms: WFM and HCS.}
\label{Table:GoldCoastResults}
\end{table*}


This section discusses the scalability of group detection in the pilot study we conduct in Gold Coast, Australia for more than one year period. We explore the feasibility of using Group-In in larger areas as opposed to relatively smaller controlled lab setups or office environments as we do in the previous section. Our goal is to see if the proposed Group-In approach is really applicable in practice to smart cities where the number of people and therefore the resulting graph size increases. %Therefore, we integrate Group-In with the setup of our city-scale pilot study.




Table~\ref{tab:Deployment} includes the information related to the Gold Coast pilot study in terms of the volume and duration of the experiment. Possible limitations of detecting groups in larger areas such as cities can be due to having many people in a city. For instance, more than 200 devices can be detected at the same time interval. This would directly result in higher data volume and larger graphs having many vertices. Moreover, since the comparison of wireless trajectories is pairwise, the number of comparisons exponentially grows with an increasing number of people. As the volume of data is larger, the latency due to querying the database may grow in a way that monitoring in real time would not be possible.  % on the aforementioned practical limitations of Group-In and include our insights from the pilot study.

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{figures/GoldCoastPhotos.pdf}
\caption{Wi-Fi scanner deployment places in Gold Coast.} %Left: shopping street, right: beach area.}
\label{Fig:Photos}
\end{figure}

Fig.~\ref{Fig:Deployment} shows the deployment locations of 17 Wi-Fi scanners in Gold Coast and Fig.~\ref{Fig:Photos} shows two of the Wi-Fi deployment positions, one on the pedestrian shopping street and another near the beach area. The crowdedness level changes during the day and based on different weekdays. The region is divided into two clusters where separate virtual machines are dedicated: Cluster 1 in the area with expected heavy pedestrian traffic (shopping street and beach area) and Cluster 2 in the area with expected light pedestrian traffic. We test Group-In for all time (including night times) where people are present in more or fewer numbers. %Even though there exist many people, Group-In works fast and efficient without any significant latency.




 \begin{figure}
\centering
\begin{minipage}{.23\textwidth}
  \centering
  \includegraphics[width=1.05\linewidth]{figures/results/AustraliaGraphOne.pdf}
        \captionof{figure}{Distribution of groups by group size observed in Cluster 1.}
                \label{fig:austfirst}
\end{minipage}\hfill
\begin{minipage}{.22\textwidth}
  \centering
  \includegraphics[width=1.03\linewidth]{figures/results/AustraliaGraphTwo.pdf}
        \captionof{figure}{The number of people and groups observed in Cluster 1.}
                \label{fig:austsecond}
\end{minipage}
\end{figure}


Fig.~\ref{fig:austfirst} and Fig.~\ref{fig:austsecond} include observations of Group-In for 1 week period ($\Delta t=30$~sec sampling time and $T=10$~min time interval). We apply WFM and HCS with pretrained (fixed) parameter values. The relation between group size and the number of groups is given in Fig. ~\ref{fig:austfirst}. The number of groups sharply decreases with the increase in group size. Moreover, the relation between the number of groups and the number of detected people is shown in Fig.~\ref{fig:austsecond}. In this figure, each time unit corresponds to a time interval ($T=10$~min). There exists a positive correlation between the number of groups and the number of detected people and the data has a daily trend with a peak value (up to 110 people) every day.


Table~\ref{Table:GoldCoastResults} shows the scalability results considering different time intervals from 2~min to 60~min of smaller-size Cluster 2 and larger-size Cluster 1. The number of people detected at each time interval, database (DB) query time, and the total group detection time (which includes both query and computation) are listed in this table. For instance, for $T=10$~min, the time it takes to create the group detection outputs is only a few seconds (for Cluster 1 having around 80 people). Therefore, the system is able to operate as a stream-based service for city-wide group monitoring. The results give us further confidence to apply Group-In in the future to even larger cities and support real-time group detection. The results from the Gold Coast pilot are monitored in the live web interface shown in Fig.~\ref{Fig:WebInterface}. Group-In analyzes the data from Gold Coast for long time periods and creates various group monitoring statistics.
